SIMDive: Approximate SIMD Soft Multiplier-Divider for FPGAs with Tunable Accuracy

The ever-increasing quest for data-level parallelism and variable precision in ubiquitous multimedia and Deep Neural Network (DNN) applications has motivated the use of Single Instruction, Multiple Data (SIMD) architectures. To alleviate energy as their main resource constraint, approximate computing has re-emerged,albeit mainly specialized for their Application-Specific Integrated Circuit (ASIC) implementations. This paper, presents for the first time, an SIMD architecture based on novel multiplier and divider with tunable accuracy, targeted for Field-Programmable Gate Arrays (FPGAs). The proposed hybrid architecture implements Mitchell's algorithms and supports precision variability from 8 to 32 bits. Experimental results obtained from Vivado, multimedia and DNN applications indicate superiority of proposed architecture (both SISD and SIMD) over accurate and state-of-the-art approximate counterparts. In particular, the proposed SISD divider outperforms the accurate Intellectual Property (IP) divider provided by Xilinx with 4x higher speed and 4.6x less energy and tolerating only < 0.8% error. Moreover, the proposed SIMD multiplier-divider supersede accurate SIMD multiplier by achieving up to 26%, 45%, 36%, and 56% improvement in area, throughput, power, and energy, respectively.

==> background.tex <==
\section{Background and Related Work}
\label{sec:relwork}
In~\secref{sec:intro} you talked about the project at a very high-level. This is
the section from where you will start giving details. First with things that are
already done, and familiarize the reader with background information they will
need to understand you work. 


\paragraph{Threat model.}
Often this section you will discuss the threat-model, but there is no strict consensus on that. 


Here is how you cite papers. For example, we read papers in the
class~\cite{rahul2016pwtypos,dodisetal:2004}.  And here is some random citation~\cite{Bojinov:2010:KLP,schechter:2010:pen,everspaugh2015pythia,bellare2009format,Juels:2014}


\subsection{Overview of the design}
\label{sec:overview}

And then just to showoff some \LaTeX skills, here is a Tikz plot.
\input{images/mainflow.tex}

You refer to a figure in the following way. In~\figref{fig:mainflow} we show
some thing that is relevant for the Multisketch paper by Chatterjee et
al.~\cite{chatterjee2019multisketches}. Add your bibliography to the
\textsf{bib.bib} file. You can copy the Bibtex format citation from Google
Scholar.

